An Ising Machine Formulation for Design Updates in Topology Optimization of Flow Channels

Topology optimization is an essential tool in computational engineering, for example, to improve the design and efficiency of flow channels. At the same time, Ising machines, including digital or quantum annealers, have been used as efficient solvers for combinatorial optimization problems. Beyond combinatorial optimization, recent works have demonstrated applicability to other engineering tasks by tailoring corresponding problem formulations. In this study, we present a novel Ising machine formulation for computing design updates during topology optimization with the goal of minimizing dissipation energy in flow channels. We explore the potential of this approach to improve the efficiency and performance of the optimization process. To this end, we conduct experiments to study the impact of various factors within the novel formulation. Additionally, we compare it to a classical method using the number of optimization steps and the final values of the objective function as indicators of the time intensity of the optimization and the performance of the resulting designs, respectively. Our findings show that the proposed update strategy can accelerate the topology optimization process while producing comparable designs. However, it tends to be less exploratory, which may lead to lower performance of the designs. These results highlight the potential of incorporating Ising formulations for optimization tasks but also show their limitations when used to compute design updates in an iterative optimization process. In conclusion, this work provides an efficient alternative for design updates in topology optimization and enhances the understanding of integrating Ising machine formulations in engineering optimization.

==> fig/parameter_study/diffuser/regularization/0/char_func.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={Characteristic Function},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/0/char_func-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {char_func-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/0/level_set.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=-1,
tick align=outside,
tick pos=left,
title={Level-Set},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/0/level_set-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {level_set-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/1/char_func.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={Characteristic Function},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/1/char_func-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {char_func-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/1/level_set.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=-1,
tick align=outside,
tick pos=left,
title={Level-Set},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/1/level_set-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {level_set-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/2/char_func.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={Characteristic Function},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/2/char_func-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {char_func-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/2/level_set.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=-1,
tick align=outside,
tick pos=left,
title={Level-Set},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/2/level_set-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {level_set-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/3/char_func.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={Characteristic Function},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/3/char_func-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {char_func-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/3/level_set.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=0.777777777777778,
point meta min=-1,
tick align=outside,
tick pos=left,
title={Level-Set},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/3/level_set-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {level_set-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/4/char_func.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={Characteristic Function},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/4/char_func-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {char_func-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularization/4/level_set.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap/blackwhite,
point meta max=0.777777777777778,
point meta min=-0.777777777777778,
tick align=outside,
tick pos=left,
title={Level-Set},
x grid style={darkgray176},
xlabel={x},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={y},
ymin=0, ymax=1,
ytick style={color=black}
]
<<<<<<< HEAD
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {fig/parameter_study/diffuser/regularization/4/level_set-000.png};
=======
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {level_set-000.png};
>>>>>>> 5844b79 (Update figures for study of regularization effect on level-set and char func)
\end{axis}

\end{tikzpicture}


==> fig/parameter_study/diffuser/regularizationDissipation/dis_reg_modified.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}%[font=\normalsize]

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{groupplot}[group style={group size=5 by 5, horizontal sep=10pt, vertical sep=10pt},height=80pt,width=80pt]
\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={0.0},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-000.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-001.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-002.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-003.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-004.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={25.0},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-005.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-006.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-007.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-008.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-009.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={50.0},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-010.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-011.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-012.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-013.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-014.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={75.0},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-015.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-016.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-017.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-018.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-019.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xlabel={0.0},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={100.0},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-020.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xlabel={1.0},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-021.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xlabel={2.0},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-022.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xlabel={3.0},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-023.png};

\nextgroupplot[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xlabel={4.0},
xmajorticks=false,
xmin=-0.5, xmax=31.5,
xtick style={color=black},
xticklabels={},
y dir=reverse,
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.5, ymax=31.5,
ytick style={color=black},
yticklabels={}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=31.5, ymin=31.5, ymax=-0.5] {fig/parameter_study/diffuser/regularizationDissipation/dis_reg-024.png};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!-0.02!(current bounding box.north west)$}) node[
  scale=1.0,
  anchor=base,
  text=black,
  rotate=0.0
]{$\lambda_{\mathrm{reg}}\longrightarrow$};
\draw ({$(current bounding box.south west)!-0.02!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=1.0,
  anchor=west,
  text=black,
  rotate=90.0
]{$\longleftarrow\lambda_{\mathrm{dis}}$};
\end{tikzpicture}

